iFlipper: Label Flipping for Individual Fairness

As machine learning becomes prevalent, mitigating any unfairness present in the training data becomes critical. Among the various notions of fairness, this paper focuses on the well-known individual fairness, which states that similar individuals should be treated similarly. While individual fairness can be improved when training a model (in-processing), we contend that fixing the data before model training (pre-processing) is a more fundamental solution. In particular, we show that label flipping is an effective pre-processing technique for improving individual fairness. Our system iFlipper solves the optimization problem of minimally flipping labels given a limit to the individual fairness violations, where a violation occurs when two similar examples in the training data have different labels. We first prove that the problem is NP-hard. We then propose an approximate linear programming algorithm and provide theoretical guarantees on how close its result is to the optimal solution in terms of the number of label flips. We also propose techniques for making the linear programming solution more optimal without exceeding the violations limit. Experiments on real datasets show that iFlipper significantly outperforms other pre-processing baselines in terms of individual fairness and accuracy on unseen test sets. In addition, iFlipper can be combined with in-processing techniques for even better results.

==> futurework.tex <==
\section{Discussion and Future Work} \label{sec:futurework}
\rev{
We believe pre-processing is important to mitigate model fairness as the data is the root cause of unfairness, and that there needs to be more emphasis on pre-processing research including \systems{}. Below are some possible directions for improving \systems{}.

\paragraph*{Multi-class Classification and Regression Tasks} 
\systems{} currently solves binary classification problems, and we would like to support multi-class classification and regression tasks in our future work. For multi-class classification, we can either group the labels to favorable and unfavorable labels and make the problem a binary classification one. Alternatively, we can solve a one-vs-all problem for each class (binary classification) and use a softmax to calculate the final label. For regression, the action becomes changing the label instead of flipping it. Since the current optimization problem can be extended to support continuous labels, we should be able to change the optimization setup to support regression problems. However, we need to derived the theoretical proof of feasibility and the study of optimality of the LP solution on these two settings.



% \paragraph*{Applicability to Group Fairness} 
% Kamiran et al.~\cite{kamiran2012data} proposed a label flipping technique to improve statistical parity, which is one of the group fairness measures. 
}
